Temporal Graph Network Embedding with Causal Anonymous Walks Representations

Many tasks in graph machine learning, such as link prediction and node classification, are typically solved by using representation learning, in which each node or edge in the network is encoded via an embedding. Though there exists a lot of network embeddings for static graphs, the task becomes much more complicated when the dynamic (i.e. temporal) network is analyzed. In this paper, we propose a novel approach for dynamic network representation learning based on Temporal Graph Network by using a highly custom message generating function by extracting Causal Anonymous Walks. For evaluation, we provide a benchmark pipeline for the evaluation of temporal network embeddings. This work provides the first comprehensive comparison framework for temporal network representation learning in every available setting for graph machine learning problems involving node classification and link prediction. The proposed model outperforms state-of-the-art baseline models. The work also justifies the difference between them based on evaluation in various transductive/inductive edge/node classification tasks. In addition, we show the applicability and superior performance of our model in the real-world downstream graph machine learning task provided by one of the top European banks, involving credit scoring based on transaction data.

==> 7_1_fin_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Enron}}     & \textbf{10\% and 75\%}  & $0.563 \pm 0.116$ & $0.522 \pm 0.043$ & $0.55 \pm 0.042$  & $0.643 \pm 0.024$  \\
                                    & \textbf{75\% and 10\%}  & $0.415 \pm 0.04$  & $0.688 \pm 0.058$ & $0.693 \pm 0.043$ & $0.742 \pm 0.028$  \\
                                    & \textbf{75\% and 75\%}  & $0.443 \pm 0.063$ & $0.695 \pm 0.044$ & $0.681 \pm 0.075$ & $0.709 \pm 0.026$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Ethereum}}  & \textbf{10\% and 75\%}  & $0.53 \pm 0.006$  & $0.658 \pm 0.051$ & $0.648 \pm 0.032$ & $0.656 \pm 0.035$  \\
                                    & \textbf{75\% and 10\%}  & $0.503 \pm 0.002$ & $0.638 \pm 0.011$ & $0.619 \pm 0.011$ & $0.645 \pm 0.007$  \\
                                    & \textbf{75\% and 75\%}  & $0.505 \pm 0.007$ & $0.633 \pm 0.01$  & $0.612 \pm 0.019$ & $0.634 \pm 0.01$   \\ \cline{1-1}
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.565 \pm 0.054$ & $0.827 \pm 0.012$ & $0.83 \pm 0.013$  & $0.842 \pm 0.01$   \\
                                    & \textbf{75\% and 10\%}  & $0.452 \pm 0.127$ & $0.932 \pm 0.004$ & $0.924 \pm 0.0$   & $0.934 \pm 0.004$  \\
                                    & \textbf{75\% and 75\%}  & $0.463 \pm 0.117$ & $0.924 \pm 0.005$ & $0.912 \pm 0.008$ & $0.919 \pm 0.004$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{UCI}}       & \textbf{10\% and 75\%}  & $0.529 \pm 0.028$ & $0.646 \pm 0.019$ & $0.644 \pm 0.028$ & $0.664 \pm 0.006$  \\
                                    & \textbf{75\% and 10\%}  & $0.495 \pm 0.02$  & $0.782 \pm 0.013$ & $0.767 \pm 0.01$  & $0.763 \pm 0.006$  \\
                                    & \textbf{75\% and 75\%}  & $0.486 \pm 0.018$ & $0.785 \pm 0.018$ & $0.775 \pm 0.015$ & $0.763 \pm 0.009$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.534 \pm 0.033$ & $0.943 \pm 0.009$ & $0.932 \pm 0.013$ & $0.95 \pm 0.003$   \\
                                    & \textbf{75\% and 10\%}  & $0.468 \pm 0.013$ & $0.904 \pm 0.008$ & $0.896 \pm 0.015$ & $0.916 \pm 0.009$  \\
                                    & \textbf{75\% and 75\%}  & $0.476 \pm 0.014$ & $0.902 \pm 0.012$ & $0.888 \pm 0.014$ & $0.908 \pm 0.005$ 
\end{tabular}
\caption{Inductive edge prediction results, AP}
\label{tab:edge_ind_ap}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Enron}}     & \textbf{10\% and 75\%}  & $0.501 \pm 0.218$ & $0.384 \pm 0.078$ & $0.416 \pm 0.087$ & $0.616 \pm 0.041$  \\
                                    & \textbf{75\% and 10\%}  & $0.359 \pm 0.064$ & $0.697 \pm 0.055$ & $0.693 \pm 0.038$ & $0.74 \pm 0.03$    \\
                                    & \textbf{75\% and 75\%}  & $0.398 \pm 0.093$ & $0.706 \pm 0.041$ & $0.687 \pm 0.074$ & $0.698 \pm 0.024$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Ethereum}}  & \textbf{10\% and 75\%}  & $0.519 \pm 0.012$ & $0.677 \pm 0.064$ & $0.665 \pm 0.048$ & $0.679 \pm 0.049$  \\
                                    & \textbf{75\% and 10\%}  & $0.483 \pm 0.002$ & $0.656 \pm 0.018$ & $0.629 \pm 0.019$ & $0.667 \pm 0.011$  \\
                                    & \textbf{75\% and 75\%}  & $0.494 \pm 0.014$ & $0.654 \pm 0.013$ & $0.616 \pm 0.031$ & $0.654 \pm 0.011$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.581 \pm 0.055$ & $0.788 \pm 0.019$ & $0.795 \pm 0.018$ & $0.812 \pm 0.012$  \\
                                    & \textbf{75\% and 10\%}  & $0.362 \pm 0.151$ & $0.92 \pm 0.004$  & $0.91 \pm 0.0$    & $0.923 \pm 0.005$  \\
                                    & \textbf{75\% and 75\%}  & $0.375 \pm 0.137$ & $0.913 \pm 0.007$ & $0.897 \pm 0.01$  & $0.906 \pm 0.003$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{UCI}}       & \textbf{10\% and 75\%}  & $0.546 \pm 0.019$ & $0.58 \pm 0.023$  & $0.58 \pm 0.034$  & $0.596 \pm 0.01$   \\
                                    & \textbf{75\% and 10\%}  & $0.485 \pm 0.026$ & $0.745 \pm 0.017$ & $0.723 \pm 0.017$ & $0.718 \pm 0.011$  \\
                                    & \textbf{75\% and 75\%}  & $0.468 \pm 0.025$ & $0.75 \pm 0.021$  & $0.734 \pm 0.021$ & $0.725 \pm 0.008$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.571 \pm 0.037$ & $0.936 \pm 0.009$ & $0.925 \pm 0.014$ & $0.949 \pm 0.004$  \\
                                    & \textbf{75\% and 10\%}  & $0.448 \pm 0.02$  & $0.895 \pm 0.011$ & $0.887 \pm 0.016$ & $0.906 \pm 0.011$  \\
                                    & \textbf{75\% and 75\%}  & $0.46 \pm 0.025$  & $0.891 \pm 0.013$ & $0.881 \pm 0.015$ & $0.896 \pm 0.008$ 
\end{tabular}
\caption{Inductive edge prediction results, AUC}
\label{tab:edge_ind_auc}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Enron}}     & \textbf{10\% and 75\%}  & $0.513 \pm 0.032$ & $0.698 \pm 0.039$ & $0.677 \pm 0.067$ & $0.693 \pm 0.034$  \\
                                    & \textbf{75\% and 10\%}  & $0.493 \pm 0.043$ & $0.73 \pm 0.059$  & $0.74 \pm 0.062$  & $0.736 \pm 0.038$  \\
                                    & \textbf{75\% and 75\%}  & $0.487 \pm 0.04$  & $0.723 \pm 0.059$ & $0.699 \pm 0.063$ & $0.694 \pm 0.031$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Ethereum}}  & \textbf{10\% and 75\%}  & $0.733 \pm 0.003$ & $0.93 \pm 0.003$  & $0.916 \pm 0.005$ & $0.931 \pm 0.002$  \\
                                    & \textbf{75\% and 10\%}  & $0.846 \pm 0.005$ & $0.932 \pm 0.002$ & $0.927 \pm 0.002$ & $0.933 \pm 0.001$  \\
                                    & \textbf{75\% and 75\%}  & $0.734 \pm 0.007$ & $0.931 \pm 0.003$ & $0.92 \pm 0.006$  & $0.932 \pm 0.003$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.648 \pm 0.057$ & $0.978 \pm 0.002$ & $0.969 \pm 0.006$ & $0.976 \pm 0.001$  \\
                                    & \textbf{75\% and 10\%}  & $0.734 \pm 0.066$ & $0.981 \pm 0.002$ & $0.974 \pm 0.0$   & $0.976 \pm 0.001$  \\
                                    & \textbf{75\% and 75\%}  & $0.649 \pm 0.069$ & $0.978 \pm 0.001$ & $0.966 \pm 0.007$ & $0.96 \pm 0.013$   \\ \cline{1-1}
\multirow{3}{*}{\textbf{UCI}}       & \textbf{10\% and 75\%}  & $0.5 \pm 0.014$   & $0.792 \pm 0.016$ & $0.762 \pm 0.048$ & $0.813 \pm 0.009$  \\
                                    & \textbf{75\% and 10\%}  & $0.558 \pm 0.012$ & $0.743 \pm 0.024$ & $0.7 \pm 0.046$   & $0.778 \pm 0.028$  \\
                                    & \textbf{75\% and 75\%}  & $0.501 \pm 0.021$ & $0.789 \pm 0.021$ & $0.768 \pm 0.04$  & $0.79 \pm 0.031$   \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.695 \pm 0.041$ & $0.97 \pm 0.003$  & $0.966 \pm 0.003$ & $0.969 \pm 0.003$  \\
                                    & \textbf{75\% and 10\%}  & $0.684 \pm 0.038$ & $0.975 \pm 0.002$ & $0.969 \pm 0.004$ & $0.972 \pm 0.002$  \\
                                    & \textbf{75\% and 75\%}  & $0.697 \pm 0.017$ & $0.969 \pm 0.005$ & $0.964 \pm 0.007$ & $0.969 \pm 0.003$ 
\end{tabular}
\caption{Transductive edge prediction results, AP}
\label{tab:edge_tra_AP}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Enron}}     & \textbf{10\% and 75\%}  & $0.541 \pm 0.037$ & $0.7 \pm 0.043$   & $0.679 \pm 0.068$ & $0.688 \pm 0.035$  \\
                                    & \textbf{75\% and 10\%}  & $0.498 \pm 0.081$ & $0.726 \pm 0.059$ & $0.738 \pm 0.066$ & $0.738 \pm 0.047$  \\
                                    & \textbf{75\% and 75\%}  & $0.492 \pm 0.072$ & $0.721 \pm 0.059$ & $0.699 \pm 0.069$ & $0.687 \pm 0.037$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Ethereum}}  & \textbf{10\% and 75\%}  & $0.728 \pm 0.005$ & $0.932 \pm 0.004$ & $0.914 \pm 0.008$ & $0.933 \pm 0.002$  \\
                                    & \textbf{75\% and 10\%}  & $0.868 \pm 0.005$ & $0.936 \pm 0.002$ & $0.929 \pm 0.003$ & $0.937 \pm 0.002$  \\
                                    & \textbf{75\% and 75\%}  & $0.73 \pm 0.008$  & $0.934 \pm 0.003$ & $0.919 \pm 0.008$ & $0.934 \pm 0.003$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.663 \pm 0.049$ & $0.978 \pm 0.002$ & $0.969 \pm 0.006$ & $0.976 \pm 0.001$  \\
                                    & \textbf{75\% and 10\%}  & $0.73 \pm 0.065$  & $0.98 \pm 0.002$  & $0.973 \pm 0.0$   & $0.976 \pm 0.001$  \\
                                    & \textbf{75\% and 75\%}  & $0.658 \pm 0.073$ & $0.978 \pm 0.001$ & $0.966 \pm 0.007$ & $0.958 \pm 0.014$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{UCI}}       & \textbf{10\% and 75\%}  & $0.498 \pm 0.019$ & $0.768 \pm 0.019$ & $0.729 \pm 0.063$ & $0.786 \pm 0.015$  \\
                                    & \textbf{75\% and 10\%}  & $0.572 \pm 0.019$ & $0.701 \pm 0.025$ & $0.652 \pm 0.062$ & $0.744 \pm 0.028$  \\
                                    & \textbf{75\% and 75\%}  & $0.497 \pm 0.021$ & $0.762 \pm 0.025$ & $0.737 \pm 0.055$ & $0.761 \pm 0.035$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.72 \pm 0.036$  & $0.968 \pm 0.003$ & $0.963 \pm 0.003$ & $0.967 \pm 0.003$  \\
                                    & \textbf{75\% and 10\%}  & $0.711 \pm 0.039$ & $0.973 \pm 0.002$ & $0.967 \pm 0.005$ & $0.97 \pm 0.002$   \\
                                    & \textbf{75\% and 75\%}  & $0.718 \pm 0.014$ & $0.967 \pm 0.004$ & $0.961 \pm 0.007$ & $0.967 \pm 0.003$ 
\end{tabular}
\caption{Transductive edge prediction results, AUC}
\label{tab:edge_tra_AUC}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.408 \pm 0.025$ & $0.553 \pm 0.034$ & $0.505 \pm 0.041$ & $0.604 \pm 0.02$   \\
                                    & \textbf{75\% and 10\%}  & $0.487 \pm 0.019$ & $0.499 \pm 0.025$ & $0.544 \pm 0.0$   & $0.546 \pm 0.03$   \\
                                    & \textbf{75\% and 75\%}  & $0.49 \pm 0.037$  & $0.522 \pm 0.05$  & $0.512 \pm 0.052$ & $0.516 \pm 0.03$   \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.755 \pm 0.073$ & $0.69 \pm 0.068$  & $0.676 \pm 0.068$ & $0.728 \pm 0.06$   \\
                                    & \textbf{75\% and 10\%}  & $0.63 \pm 0.055$  & $0.627 \pm 0.041$ & $0.623 \pm 0.034$ & $0.681 \pm 0.062$  \\
                                    & \textbf{75\% and 75\%}  & $0.63 \pm 0.068$  & $0.595 \pm 0.052$ & $0.624 \pm 0.062$ & $0.67 \pm 0.035$   \\ \cline{1-1}
\end{tabular}
\caption{Inductive node classification results, AUC}
\label{tab:node_ind_AUC}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{l|l|llll}
\textbf{Dataset}                    & \textbf{Node-edge mask} & \textbf{Jodie}    & \textbf{TGN}      & \textbf{DyRep}    & \textbf{Our model} \\ \hline
\multirow{3}{*}{\textbf{Reddit}}    & \textbf{10\% and 75\%}  & $0.5 \pm 0.045$   & $0.595 \pm 0.029$ & $0.613 \pm 0.031$ & $0.604 \pm 0.038$  \\
                                    & \textbf{75\% and 10\%}  & $0.489 \pm 0.055$ & $0.605 \pm 0.014$ & $0.601 \pm 0.0$   & $0.639 \pm 0.005$  \\
                                    & \textbf{75\% and 75\%}  & $0.503 \pm 0.059$ & $0.602 \pm 0.038$ & $0.603 \pm 0.019$ & $0.601 \pm 0.037$  \\ \cline{1-1}
\multirow{3}{*}{\textbf{Wikipedia}} & \textbf{10\% and 75\%}  & $0.852 \pm 0.012$ & $0.725 \pm 0.043$ & $0.742 \pm 0.045$ & $0.773 \pm 0.041$  \\
                                    & \textbf{75\% and 10\%}  & $0.856 \pm 0.02$  & $0.732 \pm 0.044$ & $0.762 \pm 0.047$ & $0.789 \pm 0.042$  \\
                                    & \textbf{75\% and 75\%}  & $0.852 \pm 0.015$ & $0.748 \pm 0.055$ & $0.737 \pm 0.045$ & $0.752 \pm 0.021$  \\ \cline{1-1}
\end{tabular}
\caption{Transductive node classification results, AUC}
\label{tab:node_tra_AUC}
\end{table*}

==> 9_discussion.tex <==


\section{Discussion}

The obtained results demonstrate that our model is capable of producing high-quality node embeddings for all three types of tasks. In this section we discuss details of the observed metrics.

First, we can see that no model unequivocally dominates others on all types of tasks. However, it should be noted that we were able to tune our model to outperform almost all other embedding model results. This would mean that, in case of default parameters of other models being close to optimal, we consistently outperform the other approaches.

For transductive edge prediction, we observe that our model manages to generate the best results, with the exception of a few model setups, where TGN and, in one instance, DyRep, achieve comparable or better results. This indicates that using CAW features generally offers an improvement over TGN and existing models, though in some cases the information added by incorporating CAW features may be "doubled" by other model encoding modules.

For inductive edge prediction, we observe that our method achieves best results on all datasets, with the exception of Wikipedia dataset, where on one of the setups (lean node mask, strict edge mask) TGN and DyRep show similar results. We see this as further supporting evidence of our model's enhanced ability to capture network-wide commonly occurring patterns - which are encoded by the CAW-generated features.

For node classification task, our model generally sees an improvement over existing results, indicating the high quality of obtained embeddings. One minor detail that is worthy of discussion is performance of Jodie. We can see that it outperforms our model in node classification tasks on Wikipedia dataset. We attribute it to the design of the Jodie model, which incorporates both static and dynamic node embeddings, which might have contributed to the quality of encoding interests and behavior patterns of the Wikipedia editors.

To summarize, the experimental setup, along with the ablation study, shows the applicability of our method to solving various prediction tasks on temporal networks, and, at least in some instances, significantly improving the existing results. Below, we hypothesize the reasons that allow our model to achieve this.

The modification of the message generating function can be expected to have an effect, as it provides the model with an additional way to differentiate the messages based on their relevance. NEF features of an edge contain information about the walk correlation of the two nodes; as this information is enough for inferring link prediction with high accuracy, it should contain a high descriptive value. This could, for instance, allow the model to classify some messages as being more random and irrelevant, and diminish their effect on the memory update.

Similar reasoning works to justify the modification of the embedding module. While the original version of this module allows treating k-hop neighbors of the node differently when using attention for aggregation, it might be beneficial to enhance  the model with NEF features of connections between the node and its closest neighbors. This way, we add the information about walk correlation between the node and the neighbor and allow the model to better account for differences in neighborhood types.

